Mastering Atari 2600 Games with Discovered Options

Temporal abstractions, often instantiated as options, have long been regarded as a mechanism for accelerating credit assignment, facilitating exploration, and enabling generalisation in reinforcement learning (RL). However, developing general option discovery methods that are effective in large-scale, high-dimensional domains remains a fundamental challenge. Existing option discovery methods are either confined to relatively simple domains, depend on handcrafted or quasi-symbolic representations, or offer little improvement over learning without options. We present Wayfarer, a general, domain-agnostic, online deep RL agent that discovers options through Laplacian representation learning from high-dimensional observations and leverages them for control. We show that the resulting options simultaneously improve exploration, accelerate credit assignment, and generalise effectively to unseen settings, enabling substantially faster learning of complex policies. Wayfarer achieves state-of-the-art performance among single-stream agents on the most challenging Atari 2600 games, with the largest gains in games that require long-horizon exploration and strategic behaviour, such as Montezuma's Revenge and Private Eye.

==> compact-title.tex <==
    
    \makeatletter
    
    \renewcommand\metadataformat[2][]{{\textbf{#1:} #2}}
    \renewcommand\metadata[2][]{%
      \amii@addtolist[#1]{#2}{\metadatalist}{\metadataformat}{\quad}}
    
    \renewcommand\affiliationformat[2][]{{\small $^{#1}$#2}}
    
    \renewcommand{\maketitle}{%
      \thispagestyle{plain}%
      \suppressfloats[t]%
      \begin{tcolorbox}[
        enhanced, frame hidden, arc=10pt, colback=amiibg,
        boxsep=0pt,
        left=0.6cm, right=0.6cm, top=0.55cm, bottom=0.55cm,
        before skip=0pt, after skip=0.35cm
      ]
        \setlength{\parindent}{0pt}%
        \setlength{\parskip}{0pt}%
    
        \noindent
        \begin{minipage}[t]{\dimexpr\linewidth-1.9cm\relax}
          \vspace{0pt}%
          \raggedright
          \hyphenpenalty=10000
          {\setstretch{1}\huge\bfseries\color{amiinight}%
           \amii@title\par}%
        \end{minipage}\hfill
        \begin{minipage}[t]{1.75cm}
          \vspace{0pt}%
          \raggedleft
          \includegraphics[width=\linewidth]{assets/amii-logo.pdf}%
        \end{minipage}\par
    
        \vspace{0.30cm}%
        {\raggedright
          \hyphenpenalty=10000
          \authorlist\par
          \vspace{0.15cm}%
          \affiliationlist\par
          \ifdefempty{\contributionlist}{}{%
            \vspace{0.10cm}%
            \contributionlist\par}%
        }
    
        \vspace{0.45cm}%
        {\color{amiicharcoal}\abstractlist\par}%
    
        \ifdefempty{\metadatalist}{}{%
          \vspace{0.40cm}%
          {\small\raggedright\color{amiicharcoal}\metadatalist\par}%
        }%
      \end{tcolorbox}%
    }
    
    \makeatother
    

